Systematically Detecting Packet Validation Vulnerabilities in Embedded Network Stacks

Embedded Network Stacks (ENS) enable low-resource devices to communicate with the outside world, facilitating the development of the Internet of Things and Cyber-Physical Systems. Some defects in ENS are thus high-severity cybersecurity vulnerabilities: they are remotely triggerable and can impact the physical world. While prior research has shed light on the characteristics of defects in many classes of software systems, no study has described the properties of ENS defects nor identified a systematic technique to expose them. The most common automated approach to detecting ENS defects is feedback-driven randomized dynamic analysis ("fuzzing"), a costly and unpredictable technique. This paper provides the first systematic characterization of cybersecurity vulnerabilities in ENS. We analyzed 61 vulnerabilities across 6 open-source ENS. Most of these ENS defects are concentrated in the transport and network layers of the network stack, require reaching different states in the network protocol, and can be triggered by only 1-2 modifications to a single packet. We therefore propose a novel systematic testing framework that focuses on the transport and network layers, uses seeds that cover a network protocol's states, and systematically modifies packet fields. We evaluated this framework on 4 ENS and replicated 12 of the 14 reported IP/TCP/UDP vulnerabilities. On recent versions of these ENSs, it discovered 7 novel defects (6 assigned CVES) during a bounded systematic test that covered all protocol states and made up to 3 modifications per packet. We found defects in 3 of the 4 ENS we tested that had not been found by prior fuzzing research. Our results suggest that fuzzing should be deferred until after systematic testing is employed.

==> design.tex <==
\begin{figure*}

\label{fig:fig-design-overviw-old}

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,411); %set diagram left start at 0, and has height of 411

%Straight Lines [id:da3025139260822869] 
\draw    (100,190) -- (100,238) ;
\draw [shift={(100,240)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9482070503551627] 
\draw    (140,270) -- (238,270) ;
\draw [shift={(240,270)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da08077833398532386] 
\draw    (280,240) -- (280,132) ;
\draw [shift={(280,130)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp036572823927680465] 
\draw   (60,240) -- (140,240) -- (140,290) -- (60,290) -- cycle ;
%Shape: Rectangle [id:dp1941188523866194] 
\draw   (240,240) -- (320,240) -- (320,290) -- (240,290) -- cycle ;
%Shape: Rectangle [id:dp25107205758134166] 
\draw   (240,80) -- (320,80) -- (320,130) -- (240,130) -- cycle ;
%Shape: Rectangle [id:dp6813255743831393] 
\draw   (410,150) -- (490,150) -- (490,200) -- (410,200) -- cycle ;
%Shape: Rectangle [id:dp8299687302447113] 
\draw   (410,10) -- (490,10) -- (490,60) -- (410,60) -- cycle ;
%Shape: Rectangle [id:dp47407247701553745] 
\draw   (570,60) -- (650,60) -- (650,110) -- (570,110) -- cycle ;
%Shape: Rectangle [id:dp9300619241997978] 
\draw   (570,110) -- (650,110) -- (650,160) -- (570,160) -- cycle ;
%Straight Lines [id:da04323528279183875] 
\draw    (320,100) -- (408.34,41.11) ;
\draw [shift={(410,40)}, rotate = 146.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da04363850971631589] 
\draw    (320,110) -- (408.42,178.77) ;
\draw [shift={(410,180)}, rotate = 217.87] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7209128701358599] 
\draw    (490,50) -- (568.21,89.11) ;
\draw [shift={(570,90)}, rotate = 206.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6844834575251131] 
\draw    (490,180) -- (568.3,131.06) ;
\draw [shift={(570,130)}, rotate = 147.99] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7239709571722536] 
\draw    (320,260) -- (600,260) -- (600,162) ;
\draw [shift={(600,160)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da07247631084163508] 
\draw    (620,160) -- (620,280) -- (346.33,280) -- (322,280) ;
\draw [shift={(320,280)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw  [draw opacity=0]  (58,238) -- (142,238) -- (142,292) -- (58,292) -- cycle  ;
\draw (100,265) node   [align=left] {\begin{minipage}[lt]{54.4pt}\setlength\topsep{0pt}
Test script generator
\end{minipage}};
% Text Node
\draw  [draw opacity=0]  (238,238) -- (322,238) -- (322,292) -- (238,292) -- cycle  ;
\draw (280,265) node   [align=left] {\begin{minipage}[lt]{54.4pt}\setlength\topsep{0pt}
Test executor
\end{minipage}};
% Text Node
\draw  [draw opacity=0]  (238,78) -- (322,78) -- (322,132) -- (238,132) -- cycle  ;
\draw (280,105) node   [align=left] {\begin{minipage}[lt]{54.4pt}\setlength\topsep{0pt}
Packetdrill ++
\end{minipage}};
% Text Node
\draw  [draw opacity=0]  (408,8) -- (492,8) -- (492,62) -- (408,62) -- cycle  ;
\draw (450,35) node   [align=left] {\begin{minipage}[lt]{54.4pt}\setlength\topsep{0pt}
RTOS Bridge
\end{minipage}};
% Text Node
\draw  [draw opacity=0]  (408,148) -- (492,148) -- (492,202) -- (408,202) -- cycle  ;
\draw (450,175) node   [align=left] {\begin{minipage}[lt]{54.4pt}\setlength\topsep{0pt}
Packet\\Mutator
\end{minipage}};
% Text Node
\draw  [draw opacity=0]  (568,58) -- (652,58) -- (652,112) -- (568,112) -- cycle  ;
\draw (610,85) node   [align=left] {\begin{minipage}[lt]{54.4pt}\setlength\topsep{0pt}
Test \\Agent
\end{minipage}};
% Text Node
\draw  [draw opacity=0]  (568,108) -- (652,108) -- (652,162) -- (568,162) -- cycle  ;
\draw (610,135) node   [align=left] {\begin{minipage}[lt]{54.4pt}\setlength\topsep{0pt}
RTOS +\\Net Stack
\end{minipage}};
% Text Node
\draw (21,190) node [anchor=north west][inner sep=0.75pt]   [align=left] {Script\\Templates};
% Text Node
\draw (151,272) node [anchor=north west][inner sep=0.75pt]   [align=left] {Packetdrill\\Scripts};
% Text Node
\draw (201,172) node [anchor=north west][inner sep=0.75pt]   [align=left] {Packetdrill\\Scripts};
% Text Node
\draw (411,242) node [anchor=north west][inner sep=0.75pt]   [align=left] {Invokes};
% Text Node
\draw (401,282) node [anchor=north west][inner sep=0.75pt]   [align=left] {Crashes + hangs};
% Text Node
\draw (501,32) node [anchor=north west][inner sep=0.75pt]   [align=left] {Syscalls};
% Text Node
\draw (511,162) node [anchor=north west][inner sep=0.75pt]   [align=left] {Mutated\\Packets};


\end{tikzpicture}


\captionof{figure}{
  Figure showing the components of \fuzzername.
  The testscript generator generates test scripts with mutation instructions.
  The test executor executes Packetdrill++ and the test agent.
  RTOS bridge and Packet mutator facilitates adversarial testing of the network stack.
  The test agent wraps the network stack and delivers system calls and mutated packets to the stack.
  \JD{Not all of our stacks are RTOS, please generalize it.}
  \JD{I don't understand the relationship between Test executor and the stack under test. It is ``invoking'' the stack, but also packetdrill is directly sending syscalls/packets? What does this mean?} 
  }

\end{figure*}

==> graphics/design-overview.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,372); %set diagram left start at 0, and has height of 372

%Shape: Rectangle [id:dp046747303080719504] 
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=0.25 ] (10,10) -- (250,10) -- (250,155) -- (10,155) -- cycle ;
%Straight Lines [id:da27651437281095015] 
\draw    (120,25) -- (130,35) ;
%Straight Lines [id:da7018120120329493] 
\draw    (130,55) -- (120,65) ;
%Straight Lines [id:da5041716812689025] 
\draw    (130,25) -- (140,35) ;
%Straight Lines [id:da8333653762597261] 
\draw    (140,55) -- (130,65) ;
%Straight Lines [id:da6502679523060104] 
\draw    (90,55) -- (90,98) ;
\draw [shift={(90,100)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6819459852025139] 
\draw    (110,120) -- (178,120) ;
\draw [shift={(180,120)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp6524758982792234] 
\draw  [fill={rgb, 255:red, 168; green, 207; blue, 255 }  ,fill opacity=1 ] (60,100) -- (110,100) -- (110,130) -- (60,130) -- cycle ;
%Straight Lines [id:da03313048491971893] 
\draw    (220,120) -- (240,120) -- (240,30) -- (348,30) ;
\draw [shift={(350,30)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Polygon [id:ds30857584981670005] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.25 ] (10,175) -- (220,175) -- (220,325) -- (10,325) -- cycle ;
%Shape: Circle [id:dp9795217737988307] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (80,205) .. controls (80,202.24) and (82.24,200) .. (85,200) .. controls (87.76,200) and (90,202.24) .. (90,205) .. controls (90,207.76) and (87.76,210) .. (85,210) .. controls (82.24,210) and (80,207.76) .. (80,205) -- cycle ;
%Shape: Ellipse [id:dp1255248503929025] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (81.49,250.14) .. controls (81.49,248.05) and (83.19,246.35) .. (85.28,246.35) .. controls (87.37,246.35) and (89.06,248.05) .. (89.06,250.14) .. controls (89.06,252.23) and (87.37,253.92) .. (85.28,253.92) .. controls (83.19,253.92) and (81.49,252.23) .. (81.49,250.14) -- cycle ;
%Shape: Circle [id:dp7596594533660005] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (104.2,261.49) .. controls (104.2,259.4) and (105.9,257.71) .. (107.99,257.71) .. controls (110.08,257.71) and (111.77,259.4) .. (111.77,261.49) .. controls (111.77,263.58) and (110.08,265.28) .. (107.99,265.28) .. controls (105.9,265.28) and (104.2,263.58) .. (104.2,261.49) -- cycle ;
%Shape: Ellipse [id:dp9215059751507324] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (66.35,295.56) .. controls (66.35,293.47) and (68.05,291.77) .. (70.14,291.77) .. controls (72.23,291.77) and (73.92,293.47) .. (73.92,295.56) .. controls (73.92,297.65) and (72.23,299.34) .. (70.14,299.34) .. controls (68.05,299.34) and (66.35,297.65) .. (66.35,295.56) -- cycle ;
%Shape: Ellipse [id:dp6191787376777973] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (58.78,257.71) .. controls (58.78,255.62) and (60.48,253.92) .. (62.57,253.92) .. controls (64.66,253.92) and (66.35,255.62) .. (66.35,257.71) .. controls (66.35,259.8) and (64.66,261.49) .. (62.57,261.49) .. controls (60.48,261.49) and (58.78,259.8) .. (58.78,257.71) -- cycle ;
%Straight Lines [id:da939193864941529] 
\draw    (90,205) -- (138,205) ;
\draw [shift={(140,205)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9211582764847408] 
\draw    (85.28,246.35) -- (85.02,212) ;
\draw [shift={(85,210)}, rotate = 89.56] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9220200916463211] 
\draw    (89.06,250.14) -- (102.6,260.29) ;
\draw [shift={(104.2,261.49)}, rotate = 216.87] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da45939573803687195] 
\draw    (107.99,265.28) .. controls (108.83,289.25) and (104.7,294.12) .. (75.73,295.48) ;
\draw [shift={(73.92,295.56)}, rotate = 357.67] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da1871721332382109] 
\draw    (62.57,261.49) .. controls (57.53,276.54) and (57.59,277.4) .. (65.59,293.97) ;
\draw [shift={(66.35,295.56)}, rotate = 244.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp0553543121139648] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (140,185) -- (210,185) -- (210,255) -- (140,255) -- cycle ;
%Straight Lines [id:da9989967386602462] 
\draw    (81.49,250.14) -- (68.14,256.81) ;
\draw [shift={(66.35,257.71)}, rotate = 333.43] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Ellipse [id:dp3688898269249178] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (73.92,272.85) .. controls (73.92,270.76) and (75.62,269.06) .. (77.71,269.06) .. controls (79.8,269.06) and (81.49,270.76) .. (81.49,272.85) .. controls (81.49,274.94) and (79.8,276.63) .. (77.71,276.63) .. controls (75.62,276.63) and (73.92,274.94) .. (73.92,272.85) -- cycle ;
%Straight Lines [id:da7210780635512107] 
\draw    (77.71,276.63) -- (71.03,289.98) ;
\draw [shift={(70.14,291.77)}, rotate = 296.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da19450225853835523] 
\draw    (66.35,257.71) -- (76.29,267.65) ;
\draw [shift={(77.71,269.06)}, rotate = 225] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp47548950450471994] 
\draw   (350,25) -- (520,25) -- (520,50) -- (350,50) -- cycle ;
%Shape: Rectangle [id:dp33187662171360865] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.25 ] (240,225) -- (450,225) -- (450,325) -- (240,325) -- cycle ;
%Shape: Rectangle [id:dp9031488731714805] 
\draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.25 ] (460,225) -- (620,225) -- (620,325) -- (460,325) -- cycle ;
%Shape: Rectangle [id:dp4661252530777953] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (250,265) -- (310,265) -- (310,285) -- (250,285) -- cycle ;
%Shape: Rectangle [id:dp6557669971327027] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (400,235) -- (440,235) -- (440,265) -- (400,265) -- cycle ;
%Shape: Rectangle [id:dp8206940439777244] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (400,285) -- (440,285) -- (440,315) -- (400,315) -- cycle ;
%Shape: Rectangle [id:dp12083077763970718] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (540,255) -- (610,255) -- (610,295) -- (540,295) -- cycle ;
%Shape: Rectangle [id:dp9795855017245159] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (570,275) -- (610,275) -- (610,295) -- (570,295) -- cycle ;
%Straight Lines [id:da18664129670920748] 
\draw    (440,50) -- (440,103) ;
\draw [shift={(440,105)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9559797137646109] 
\draw    (210,205) -- (270,205) -- (270,130) -- (398,130) ;
\draw [shift={(400,130)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da928394718891831] 
\draw    (430,155) -- (430,215) -- (270,215) -- (270,263) ;
\draw [shift={(270,265)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da7113649236598482] 
\draw    (310,275) .. controls (340.54,238.23) and (359.1,246.08) .. (398.2,245.05) ;
\draw [shift={(400,245)}, rotate = 178.11] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da3209843511642697] 
\draw    (310,275) .. controls (329.93,312.89) and (368.1,306.61) .. (398.17,305.09) ;
\draw [shift={(400,305)}, rotate = 177.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da5134950682650277] 
\draw    (440,245) .. controls (498.77,244.34) and (510,246.27) .. (538.68,264.17) ;
\draw [shift={(540,265)}, rotate = 212.18] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da5387829336724448] 
\draw    (440,305) .. controls (499.07,304.34) and (500.97,308.91) .. (538.84,285.71) ;
\draw [shift={(540,285)}, rotate = 148.39] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp589558464102713] 
\draw   (400,105) -- (480,105) -- (480,155) -- (400,155) -- cycle ;
%Shape: Polygon [id:ds06869927058307734] 
\draw  [fill={rgb, 255:red, 168; green, 207; blue, 255 }  ,fill opacity=1 ] (130,35) -- (120,45) -- (130,55) -- (65.8,55) -- (20,55) -- (20,35) -- cycle ;
%Straight Lines [id:da2390056128191348] 
\draw    (80,35) -- (80,55) ;
%Straight Lines [id:da9976120178539055] 
\draw    (110,35) -- (110,55) ;
%Shape: Polygon [id:ds06324971587576533] 
\draw  [fill={rgb, 255:red, 168; green, 207; blue, 255 }  ,fill opacity=1 ] (140,35) -- (220,35) -- (220,55) -- (140,55) -- (130,45) -- cycle ;
%Straight Lines [id:da3109006159608172] 
\draw    (160,35) -- (160,55) ;
%Straight Lines [id:da56673809916718] 
\draw    (190,35) -- (190,55) ;
%Shape: Rectangle [id:dp31393596562848936] 
\draw   (55,230) -- (115.56,230) -- (115.56,303.13) -- (55,303.13) -- cycle ;
%Straight Lines [id:da5150573426027552] 
\draw    (580,255) -- (580,215) -- (450,215) -- (450,157) ;
\draw [shift={(450,155)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp17900829044874256] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (310,150) -- (390,150) -- (390,210) -- (310,210) -- cycle ;
%Shape: Rectangle [id:dp5722444897689664] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (560,235) -- (600,235) -- (600,255) -- (560,255) -- cycle ;

% Text Node
\draw (85,115) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{34pt}\setlength\topsep{0pt}
\begin{center}
TCP Data Offset
\end{center}

\end{minipage}};
% Text Node
\draw (24,17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Network packet};
% Text Node
\draw (140,135) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{40.8pt}\setlength\topsep{0pt}
\begin{center}
Get sampled value
\end{center}

\end{minipage}};
% Text Node
\draw (182,112.4) node [anchor=north west][inner sep=0.75pt]    {$0xF0$};
% Text Node
\draw (212,82.5) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{27.2pt}\setlength\topsep{0pt}
\begin{center}
Generate mutation\\Instruction
\end{center}

\end{minipage}};
% Text Node
\draw (130,165) node  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{163.2pt}\setlength\topsep{0pt}
\begin{center}
Systematic test case generation
\end{center}

\end{minipage}};
% Text Node
\draw (60,77.5) node   [align=left] {\begin{minipage}[lt]{54.4pt}\setlength\topsep{0pt}
{\scriptsize Select one field}
\end{minipage}};
% Text Node
\draw (88,40.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$F0$};
% Text Node
\draw (141,47.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$...$};
% Text Node
\draw (114,47.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$..$};
% Text Node
\draw (168,40.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$F0$};
% Text Node
\draw (198,40.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$F0$};
% Text Node
\draw (34,40.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$F0FF$};
% Text Node
\draw (83,193.5) node   [align=left] {\begin{minipage}[lt]{47.6pt}\setlength\topsep{0pt}
\begin{center}
{\scriptsize Listen state}
\end{center}

\end{minipage}};
% Text Node
\draw (85,309.5) node  [font=\normalsize] [align=left] {\begin{minipage}[lt]{61.2pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize State diagram}
\end{center}

\end{minipage}};
% Text Node
\draw (175,220) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{47.6pt}\setlength\topsep{0pt}
0 socket(...) = 3\\+0 bind(...) = 0\\+0 listen(...) = 0\\+.1 $\displaystyle < $ ack 1 win 227
\end{minipage}};
% Text Node
\draw (420,249) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{27.2pt}\setlength\topsep{0pt}
\begin{center}
ENS Bridge
\end{center}

\end{minipage}};
% Text Node
\draw (420,298) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{27.2pt}\setlength\topsep{0pt}
\begin{center}
Packet mutator
\end{center}

\end{minipage}};
% Text Node
\draw (70.5,216.5) node   [align=left] {\begin{minipage}[lt]{78.11pt}\setlength\topsep{0pt}
{\scriptsize Select one state}
\end{minipage}};
% Text Node
\draw (115,335) node  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{142.8pt}\setlength\topsep{0pt}
\begin{center}
Statefulness
\end{center}

\end{minipage}};
% Text Node
\draw (345,335) node  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{142.8pt}\setlength\topsep{0pt}
\begin{center}
Portability
\end{center}

\end{minipage}};
% Text Node
\draw (361,29.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\{rep\ tcp\ data\_off\ 0xF0 \}$};
% Text Node
\draw (350,180) node  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{54.4pt}\setlength\topsep{0pt}
{\scriptsize ...}\\{\scriptsize  +.1 $\displaystyle < $ ack 1 win 227 }\\{\scriptsize \{rep tcp data\_off 0xF0\}}
\end{minipage}};
% Text Node
\draw (520,86) node  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{108.8pt}\setlength\topsep{0pt}
Append to template
\end{minipage}};
% Text Node
\draw (540,335) node  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{108.8pt}\setlength\topsep{0pt}
\begin{center}
Detectability
\end{center}

\end{minipage}};
% Text Node
\draw (488,237) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{27.2pt}\setlength\topsep{0pt}
\begin{center}
Socket
\end{center}

\end{minipage}};
% Text Node
\draw (491,288) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{27.2pt}\setlength\topsep{0pt}
\begin{center}
Mutated \\Packet
\end{center}

\end{minipage}};
% Text Node
\draw (375,292.5) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{47.6pt}\setlength\topsep{0pt}
Packet + \\Mutation
\end{minipage}};
% Text Node
\draw (279,274) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{35.36pt}\setlength\topsep{0pt}
Packetdrill++
\end{minipage}};
% Text Node
\draw (585,265.5) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{47.6pt}\setlength\topsep{0pt}
Test Agent
\end{minipage}};
% Text Node
\draw (592,285.5) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{13.6pt}\setlength\topsep{0pt}
ENS
\end{minipage}};
% Text Node
\draw (366,236.5) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{34pt}\setlength\topsep{0pt}
Socket()
\end{minipage}};
% Text Node
\draw (435,10) node  [font=\normalsize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{115.6pt}\setlength\topsep{0pt}
\begin{center}
Instruction statement
\end{center}

\end{minipage}};
% Text Node
\draw (440,130) node  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{54.4pt}\setlength\topsep{0pt}
\begin{center}
Test Executor
\end{center}

\end{minipage}};
% Text Node
\draw (342.5,142.5) node  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{44.2pt}\setlength\topsep{0pt}
Test script
\end{minipage}};
% Text Node
\draw (535,205) node  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{95.2pt}\setlength\topsep{0pt}
Crashes / Hangs
\end{minipage}};
% Text Node
\draw (175,269.5) node  [font=\footnotesize,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{68pt}\setlength\topsep{0pt}
\begin{center}
Stateful test template
\end{center}

\end{minipage}};
% Text Node
\draw (577,245.5) node  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{13.6pt}\setlength\topsep{0pt}
ASAN
\end{minipage}};


\end{tikzpicture}


==> graphics/layers-tcp-stack.tex <==


\tikzset{every picture/.style={line width=0.75pt}}[width=0.90\columnwidth] %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,246); %set diagram left start at 0, and has height of 246

%Shape: Rectangle [id:dp39053033560891715] 
\draw   (140,10) -- (200,10) -- (200,40) -- (140,40) -- cycle ;
%Shape: Rectangle [id:dp8639905494848115] 
\draw   (140,50) -- (230,50) -- (230,80) -- (140,80) -- cycle ;
%Shape: Rectangle [id:dp332576302403762] 
\draw   (140,90) -- (230,90) -- (230,120) -- (140,120) -- cycle ;
%Shape: Rectangle [id:dp7283393493616095] 
\draw   (140,130) -- (340,130) -- (340,160) -- (140,160) -- cycle ;
%Shape: Rectangle [id:dp7011155757022296] 
\draw   (140,170) -- (340,170) -- (340,200) -- (140,200) -- cycle ;
%Shape: Rectangle [id:dp33961265428475995] 
\draw   (210,10) -- (270,10) -- (270,40) -- (210,40) -- cycle ;
%Shape: Rectangle [id:dp23637126410501086] 
\draw   (280,10) -- (340,10) -- (340,40) -- (280,40) -- cycle ;
%Shape: Rectangle [id:dp2797305132771013] 
\draw   (250,50) -- (340,50) -- (340,80) -- (250,80) -- cycle ;
%Shape: Rectangle [id:dp901537944262273] 
\draw   (250,90) -- (340,90) -- (340,120) -- (250,120) -- cycle ;

% Text Node
\draw (170,25) node   [align=left] {\begin{minipage}[lt]{40.8pt}\setlength\topsep{0pt}
\begin{center}
HTTP
\end{center}

\end{minipage}};
% Text Node
\draw (75,65) node   [align=left] {\begin{minipage}[lt]{88.4pt}\setlength\topsep{0pt}
Transport layer
\end{minipage}};
% Text Node
\draw (75,105) node   [align=left] {\begin{minipage}[lt]{88.4pt}\setlength\topsep{0pt}
Network layer
\end{minipage}};
% Text Node
\draw (75,145) node   [align=left] {\begin{minipage}[lt]{88.4pt}\setlength\topsep{0pt}
Link layer
\end{minipage}};
% Text Node
\draw (75,185) node   [align=left] {\begin{minipage}[lt]{88.4pt}\setlength\topsep{0pt}
Physical layer
\end{minipage}};
% Text Node
\draw (75,25) node   [align=left] {\begin{minipage}[lt]{88.4pt}\setlength\topsep{0pt}
Application layer
\end{minipage}};
% Text Node
\draw (240,25) node   [align=left] {\begin{minipage}[lt]{40.8pt}\setlength\topsep{0pt}
\begin{center}
DNS
\end{center}

\end{minipage}};
% Text Node
\draw (310,25) node   [align=left] {\begin{minipage}[lt]{40.8pt}\setlength\topsep{0pt}
\begin{center}
SNMP
\end{center}

\end{minipage}};
% Text Node
\draw (185,65) node   [align=left] {\begin{minipage}[lt]{61.2pt}\setlength\topsep{0pt}
\begin{center}
TCP
\end{center}

\end{minipage}};
% Text Node
\draw (295,65) node   [align=left] {\begin{minipage}[lt]{61.2pt}\setlength\topsep{0pt}
\begin{center}
UDP
\end{center}

\end{minipage}};
% Text Node
\draw (185,105) node   [align=left] {\begin{minipage}[lt]{61.2pt}\setlength\topsep{0pt}
\begin{center}
IPv4
\end{center}

\end{minipage}};
% Text Node
\draw (240,145) node   [align=left] {\begin{minipage}[lt]{136pt}\setlength\topsep{0pt}
\begin{center}
IEEE 802.15.4 MAC
\end{center}

\end{minipage}};
% Text Node
\draw (240,185) node   [align=left] {\begin{minipage}[lt]{136pt}\setlength\topsep{0pt}
\begin{center}
Radio transmition
\end{center}

\end{minipage}};
% Text Node
\draw (295,105) node   [align=left] {\begin{minipage}[lt]{61.2pt}\setlength\topsep{0pt}
\begin{center}
IPv6
\end{center}

\end{minipage}};


\end{tikzpicture}


==> graphics/packet-representation.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,102); %set diagram left start at 0, and has height of 102

%Straight Lines [id:da6256085684674237] 
\draw    (60,40) -- (60,60) ;
%Straight Lines [id:da7698116095638294] 
\draw    (30,40) -- (160,40) ;
%Straight Lines [id:da18498493932311177] 
\draw    (150,30) -- (160,40) ;
%Straight Lines [id:da37112989016871023] 
\draw    (150,50) -- (160,60) ;
%Straight Lines [id:da12002402681635005] 
\draw    (160,60) -- (150,70) ;
%Straight Lines [id:da7524275389102354] 
\draw    (160,40) -- (150,50) ;
%Straight Lines [id:da9585250857423848] 
\draw    (30,40) -- (30,60) ;
%Straight Lines [id:da07296145100509221] 
\draw    (30,60) -- (32,60) -- (160,60) ;
%Straight Lines [id:da4175682620056209] 
\draw    (90,40) -- (90,60) ;
%Straight Lines [id:da46919526280110346] 
\draw    (120,40) -- (120,60) ;
%Straight Lines [id:da09440726430975921] 
\draw    (160,30) -- (170,40) ;
%Straight Lines [id:da280447125748716] 
\draw    (160,50) -- (170,60) ;
%Straight Lines [id:da70915780857282] 
\draw    (170,60) -- (167.35,62.65) -- (160,70) ;
%Straight Lines [id:da43556533621665305] 
\draw    (170,40) -- (160,50) ;
%Straight Lines [id:da8373341814247216] 
\draw    (200,40) -- (200,60) ;
%Straight Lines [id:da9607773408815633] 
\draw    (170,40) -- (300,40) ;
%Straight Lines [id:da37338275681380395] 
\draw    (170,60) -- (300,60) ;
%Straight Lines [id:da3958543636400169] 
\draw    (230,40) -- (230,60) ;
%Straight Lines [id:da19611806067157023] 
\draw    (260,40) -- (260,60) ;
%Straight Lines [id:da9304413523539067] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (160,70) -- (160,74.3) -- (160,90) ;
%Straight Lines [id:da6647376345694871] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (550,60) -- (550,90) ;
%Straight Lines [id:da006190770695436942] 
\draw    (290,30) -- (300,40) ;
%Straight Lines [id:da09749409369060347] 
\draw    (290,50) -- (300,60) ;
%Straight Lines [id:da1594812100618328] 
\draw    (300,60) -- (294.75,65.25) -- (290,70) ;
%Straight Lines [id:da3292807983512954] 
\draw    (300,40) -- (290,50) ;
%Straight Lines [id:da7735580632777698] 
\draw    (300,30) -- (310,40) ;
%Straight Lines [id:da3982630565134695] 
\draw    (300,50) -- (310,60) ;
%Straight Lines [id:da006554014886397952] 
\draw    (310,60) -- (300,70) ;
%Straight Lines [id:da9448628927293196] 
\draw    (310,40) -- (300,50) ;
%Straight Lines [id:da8344621946151201] 
\draw    (340,40) -- (340,60) ;
%Straight Lines [id:da6483906852450209] 
\draw    (310,40) -- (341.5,40) -- (343.75,40) -- (670,40) ;
%Straight Lines [id:da878155665964567] 
\draw    (310,60) -- (670,60) ;
%Straight Lines [id:da012070823305225464] 
\draw    (370,40) -- (370,60) ;
%Straight Lines [id:da844027458330894] 
\draw    (490,40) -- (490,60) ;
%Straight Lines [id:da5282457103811076] 
\draw    (580,40) -- (580,60) ;
%Straight Lines [id:da10641355094214022] 
\draw    (610,40) -- (610,60) ;
%Straight Lines [id:da6655063978729612] 
\draw    (430,40) -- (430,60) ;
%Straight Lines [id:da3556880206996711] 
\draw    (550,40) -- (550,60) ;
%Straight Lines [id:da36773607866419544] 
\draw    (670,40) -- (670,60) ;
%Shape: Polygon [id:ds7954010614791744] 
\draw  [fill={rgb, 255:red, 204; green, 255; blue, 255 }  ,fill opacity=1 ] (310,40) -- (340,40) -- (340,60) -- (310,60) -- (300,50) -- cycle ;
%Shape: Rectangle [id:dp9900846427201943] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (610,40) -- (670,40) -- (670,60) -- (610,60) -- cycle ;

% Text Node
\draw (36,46.4) node [anchor=north west][inner sep=0.75pt]    {$45$};
% Text Node
\draw (66,46.4) node [anchor=north west][inner sep=0.75pt]    {$00$};
% Text Node
\draw (96,46.4) node [anchor=north west][inner sep=0.75pt]    {$00$};
% Text Node
\draw (126,46.4) node [anchor=north west][inner sep=0.75pt]    {$3A$};
% Text Node
\draw (176,46.4) node [anchor=north west][inner sep=0.75pt]    {$00$};
% Text Node
\draw (206,46.4) node [anchor=north west][inner sep=0.75pt]    {$00$};
% Text Node
\draw (236,46.4) node [anchor=north west][inner sep=0.75pt]    {$00$};
% Text Node
\draw (266,46.4) node [anchor=north west][inner sep=0.75pt]    {$00$};
% Text Node
\draw (316,46.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$60$};
% Text Node
\draw (346,46.4) node [anchor=north west][inner sep=0.75pt]    {$04$};
% Text Node
\draw (379,46.4) node [anchor=north west][inner sep=0.75pt]    {$003A$};
% Text Node
\draw (439,46.4) node [anchor=north west][inner sep=0.75pt]    {$2A57$};
% Text Node
\draw (503,46.4) node [anchor=north west][inner sep=0.75pt]    {$0000$};
% Text Node
\draw (556,46.4) node [anchor=north west][inner sep=0.75pt]    {$02$};
% Text Node
\draw (586,46.4) node [anchor=north west][inner sep=0.75pt]    {$04$};
% Text Node
\draw (621,46.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$0000$};
% Text Node
\draw (51,72) node [anchor=north west][inner sep=0.75pt]   [align=left] {IPv4 Header};
% Text Node
\draw (302,74) node [anchor=north west][inner sep=0.75pt]   [align=left] {TCP Header};
% Text Node
\draw (571,72) node [anchor=north west][inner sep=0.75pt]   [align=left] {TCP Option};
% Text Node
\draw (241,11) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{111.63pt}\setlength\topsep{0pt}
\begin{center}
TCP Header length field
\end{center}

\end{minipage}};
% Text Node
\draw (603,13) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{52.99pt}\setlength\topsep{0pt}
\begin{center}
MSS Value
\end{center}

\end{minipage}};


\end{tikzpicture}

